Semantic Parsing with Dual Learning

Semantic parsing converts natural language queries into structured logical forms. The paucity of annotated training samples is a fundamental challenge in this field. In this work, we develop a semantic parsing framework with the dual learning algorithm, which enables a semantic parser to make full use of data (labeled and even unlabeled) through a dual-learning game. This game between a primal model (semantic parsing) and a dual model (logical form to query) forces them to regularize each other, and can achieve feedback signals from some prior-knowledge. By utilizing the prior-knowledge of logical form structures, we propose a novel reward signal at the surface and semantic levels which tends to generate complete and reasonable logical forms. Experimental results show that our approach achieves new state-of-the-art performance on ATIS dataset and gets competitive performance on Overnight dataset.

==> tab/ablation.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\begin{table*}[htbp]
  \centering{
  \small
    \begin{tabular}{p{11.6em}|cccccccc|c|c}
    \hline
    \textbf{Method} & \multicolumn{1}{p{1.9em}}{\textbf{Bas.}} & \multicolumn{1}{p{1.9em}}{\textbf{Blo.}} & \multicolumn{1}{p{1.9em}}{\textbf{Cal.}} & \multicolumn{1}{p{1.9em}}{\textbf{Hou.}} & \multicolumn{1}{p{1.9em}}{\textbf{Pub.}} & \multicolumn{1}{p{1.9em}}{\textbf{Rec.}} & \multicolumn{1}{p{1.9em}}{\textbf{Res.}} & \multicolumn{1}{p{1.9em}|}{\textbf{Soc.}} & \multicolumn{1}{p{1.9em}|}{\textbf{Avg.}} & \multicolumn{1}{p{2em}}{\textbf{ATIS}} \\
    \hline
    \textsc{Att} & 80.1  & 55.4  & 61.9  & 53.4  & 60.2  & 64.4  & 71.1  & 76.8  & 65.4  & 78.6  \\
    % ATTN+PSEUDO+Q & 80.1  & 59.4  & 60.1  & 52.9  & 59.6  & 66.2  & 73.8  & 79.0  & 66.4  & 78.8  \\
    % ATTN+PSEUDO+LF & 83.9  & 60.4  & 64.3  & 54.5  & 58.4  & 69.0  & 70.5  & 77.3  & 67.3  & 77.9  \\
    \textsc{Att} + \textsc{Pseudo}($\mathcal{LF}$+$\mathcal{Q}$) & 80.6  & 59.1  & 61.9  & 57.1  & 62.7  & 65.3  & 73.2  & \textbf{79.8}  & 67.5  & 78.3  \\
    % ATTN+DUAL & 82.6  & 60.2  & 72.0  & 58.7  & 66.5  & 73.6  & 74.1  & 79.3  & 70.9  & 79.5  \\
    % ATTN+DUAL+Q & 83.9  & 60.7  & 70.2  & 60.8  & 69.6  & 71.3  & 76.2  & 79.8  & 71.6  & 79.7  \\
    % ATTN+DUAL+LF & 83.4  & 61.4  & 71.4  & 59.3  & 70.2  & 73.1  & 75.3  & 78.6  & 71.6  & 80.4  \\
   \textsc{Att} + \textsc{Dual} + $\mathcal{LF}$ + $\mathcal{Q}$ & \textbf{85.4}  & \textbf{62.9}  & \textbf{73.2}  & \textbf{59.3}  & \textbf{72.0}  & \textbf{75.5}  & \textbf{75.6}  & 79.5  & \textbf{72.9}  & \textbf{81.7} \\
    \hline
    \textsc{AttPtr} & 81.1  & 58.1  & 63.1  & 48.7  & 55.3  & 69.4  & 68.4  & 77.4  & 65.2  & 84.8  \\
    % ATTNPTR+PSEUDO+Q & 82.1  & 59.6  & 61.3  & 47.6  & 57.1  & 72.2  & 69.9  & 78.4  & 66.0  & 85.0  \\
    % ATTNPTR+PSEUDO+LF & 82.4  & 59.1  & 62.5  & 54.5  & 63.4  & 71.3  & 69.6  & 77.6  & 67.5  & 86.2  \\
    \textsc{AttPtr} + \textsc{Pseudo}($\mathcal{LF}$+$\mathcal{Q}$) & 81.3  & 59.4  & 65.5  & 49.2  & 58.4  & 72.7  & 72.0  & 78.6  & 67.1  & 85.0  \\
    % ATTNPTR+DUAL & 81.8  & 60.2  & 68.5  & 57.1  & 65.2  & 72.2  & 74.1  & 79.0  & 69.8  & 86.2  \\
    % ATTNPTR+DUAL+Q & 81.6  & 60.7  & 69.6  & 61.4  & 68.9  & 74.1  & 79.8  & 80.1  & 72.0  & 86.6  \\
    % ATTNPTR+DUAL+LF & 82.6  & 62.2  & 68.5  & 62.4  & 69.6  & 73.1  & 77.4  & 79.4  & 71.9  & 87.3  \\
    \textsc{AttPtr} + \textsc{Dual} + $\mathcal{LF}$ + $\mathcal{Q}$ & \textbf{83.6}  & \textbf{62.2}  & \textbf{72.6}  & \textbf{61.9}  & \textbf{71.4}  & \textbf{75.0}  & \textbf{76.5}  & \textbf{80.4}  & \textbf{73.0}  & \textbf{86.8}  \\
    \hline
    \end{tabular}%
  }
  \caption{Semi-supervised learning experiments. The proportion of labeled data to the entire training set is 50\%. Part of the results is shown. For more details, please see Appendix \ref{app:ablation_results}.}
  \label{tab:ablation}%
\end{table*}%


==> tab/ablation_more.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\begin{table}[H]
  \centering
  \small
    \begin{tabular}{p{11em}|cccccccc|c|c}
    \hline
    \textbf{Method} & \multicolumn{1}{p{1.9em}}{\textbf{Bas.}} & \multicolumn{1}{p{1.9em}}{\textbf{Blo.}} & \multicolumn{1}{p{1.9em}}{\textbf{Cal.}} & \multicolumn{1}{p{1.9em}}{\textbf{Hou.}} & \multicolumn{1}{p{1.9em}}{\textbf{Pub.}} & \multicolumn{1}{p{1.9em}}{\textbf{Rec.}} & \multicolumn{1}{p{1.9em}}{\textbf{Res.}} & \multicolumn{1}{p{1.9em}|}{\textbf{Soc.}} & \multicolumn{1}{p{1.9em}|}{\textbf{Avg.}} & \multicolumn{1}{p{2em}}{\textbf{ATIS}} \\
    \hline
    \textsc{Att} & 80.1  & 55.4  & 61.9  & 53.4  & 60.2  & 64.4  & 71.1  & 76.8  & 65.4  & 78.6  \\
    \textsc{Att}+\textsc{Pseudo}($\mathcal{Q}$) & 80.1  & 59.4  & 60.1  & 52.9  & 59.6  & 66.2  & 73.8  & 79.0  & 66.4  & 78.8  \\
    \textsc{Att}+\textsc{Pseudo}($\mathcal{LF}$) & 83.9  & 60.4  & 64.3  & 54.5  & 58.4  & 69.0  & 70.5  & 77.3  & 67.3  & 77.9  \\
    \textsc{Att}+\textsc{Pseudo}($\mathcal{LF}$+$\mathcal{Q}$) & 80.6  & 59.1  & 61.9  & 57.1  & 62.7  & 65.3  & 73.2  & \textbf{79.8}  & 67.5  & 78.3  \\
    \textsc{Att}+\textsc{Dual} & 82.6  & 60.2  & 72.0  & 58.7  & 66.5  & 73.6  & 74.1  & 79.3  & 70.9  & 79.5  \\
    \textsc{Att}+\textsc{Dual}+$\mathcal{Q}$ & 83.9  & 60.7  & 70.2  & \textbf{60.8}  & 69.6  & 71.3  & \textbf{76.2}  & \textbf{79.8}  & 71.6  & 79.7  \\
    \textsc{Att}+\textsc{Dual}+$\mathcal{LF}$ & 83.4  & 61.4  & 71.4  & 59.3  & 70.2  & 73.1  & 75.3  & 78.6  & 71.6  & 80.4  \\
    \textsc{Att}+\textsc{Dual}+$\mathcal{LF}$+$\mathcal{Q}$ & \textbf{85.4}  & \textbf{62.9}  & \textbf{73.2}  & 59.3  & \textbf{72.0}  & \textbf{75.5}  & 75.6  & 79.5  & \textbf{72.9}  & \textbf{81.7} \\
    \hline
    \textsc{AttPtr} & 81.1  & 58.1  & 63.1  & 48.7  & 55.3  & 69.4  & 68.4  & 77.4  & 65.2  & 84.8  \\
    \textsc{AttPtr}+\textsc{Pseudo}($\mathcal{Q}$) & 82.1  & 59.6  & 61.3  & 47.6  & 57.1  & 72.2  & 69.9  & 78.4  & 66.0  & 85.0  \\
    \textsc{AttPtr}+\textsc{Pseudo}($\mathcal{LF}$) & 82.4  & 59.1  & 62.5  & 54.5  & 63.4  & 71.3  & 69.6  & 77.6  & 67.5  & 86.2  \\
    \textsc{AttPtr}+\textsc{Pseudo}($\mathcal{LF}$+$\mathcal{Q}$) & 81.3  & 59.4  & 65.5  & 49.2  & 58.4  & 72.7  & 72.0  & 78.6  & 67.1  & 85.0  \\
    \textsc{AttPtr}+\textsc{Dual} & 81.8  & 60.2  & 68.5  & 57.1  & 65.2  & 72.2  & 74.1  & 79.0  & 69.8  & 86.2  \\
    \textsc{AttPtr}+\textsc{Dual}+$\mathcal{Q}$ & 81.6  & 60.7  & 69.6  & 61.4  & 68.9  & 74.1  & \textbf{79.8}  & 80.1  & 72.0  & 86.6  \\
    \textsc{AttPtr}+\textsc{Dual}+$\mathcal{LF}$ & 82.6  & \textbf{62.2}  & 68.5  & \textbf{62.4}  & 69.6  & 73.1  & 77.4  & 79.4  & 71.9  & \textbf{87.3}  \\
    \textsc{AttPtr}+\textsc{Dual}+$\mathcal{LF}$+$\mathcal{Q}$ & \textbf{83.6}  & \textbf{62.2}  & \textbf{72.6}  & 61.9  & \textbf{71.4}  & \textbf{75.0}  & 76.5  & \textbf{80.4}  & \textbf{73.0}  & 86.8  \\
    \hline
    \end{tabular}%
  \caption{Semi-supervised learning experiments. We keep 50\% of the training set as labeled data randomly and leave the rest as unpaired queries($\mathcal{Q}$) and logical forms($\mathcal{LF}$) to simulate unsupervised dataset. \textsc{Dual} denotes training models by dual learning algorithm. \textsc{Pseudo} uses the $Q2LF$ model and $\mathcal{Q}$ to generate pseudo-labeled data, as well as $LF2Q$ model and $\mathcal{LF}$. }
  \label{tab:ablation_more}%
\end{table}%

